How Deep is your Guess? A Fresh Perspective on Deep Learning for Medical Time-Series Imputation

We present a comprehensive analysis of deep learning approaches for Electronic Health Record (EHR) time-series imputation, examining how architectural and framework biases combine to influence model performance. Our investigation reveals varying capabilities of deep imputers in capturing complex spatiotemporal dependencies within EHRs, and that model effectiveness depends on how its combined biases align with medical time-series characteristics. Our experimental evaluation challenges common assumptions about model complexity, demonstrating that larger models do not necessarily improve performance. Rather, carefully designed architectures can better capture the complex patterns inherent in clinical data. The study highlights the need for imputation approaches that prioritise clinically meaningful data reconstruction over statistical accuracy. Our experiments show imputation performance variations of up to 20\% based on preprocessing and implementation choices, emphasising the need for standardised benchmarking methodologies. Finally, we identify critical gaps between current deep imputation methods and medical requirements, highlighting the importance of integrating clinical insights to achieve more reliable imputation approaches for healthcare applications.

==> scrap.tex <==

archiectures are deterministic - stochasticity is introduced by frameworks. 
The four dimensions reflect key design choices in deep imputation models:
Modeling Approach defines the fundamental inference strategy: deterministic models produce fixed outputs,
Deterministic approaches focus on direct reconstruction of missing values through sequential and local pattern recognition.

probabilistic models capture uncertainty through distributions, and hybrid approaches combine both elements. Probabilistic models introduce a more nuanced approach to imputation by modeling data distributions and quantifying uncertainty.
Missing Data Handling describes how missing values are processed: direct imputation predicts values explicitly, generative modeling reconstructs entire distributions, and latent representation learns compressed encodings of the data patterns.
Pattern Assumptions specify how temporal relationships are modeled: sequential for ordered dependencies, global for all-to-all interactions, local for neighborhood patterns, and relational for graph-like structures.
Data Assumptions encompass statistical premises about the data: missingness mechanism (MAR/MCAR/MNAR) indicates how values become missing, distribution captures the data's probabilistic nature, temporal dependencies model time-based relationships, and variable dependencies represent interactions between features.

conclusion: 

This taxonomy illuminates the multifaceted landscape of deep learning imputation models. By understanding the interplay between modeling approaches, temporal strategies, and missing data handling mechanisms, researchers can more effectively navigate the challenges of incomplete medical time series data.

The field continues to evolve, with ongoing research focusing on enhancing model interpretability, uncertainty quantification, and clinical relevance.




\begin{table*}[!t]
\renewcommand{\arraystretch}{1.3}
\caption{Relationship Between EHR Characteristics and Deep Learning Imputation Approaches}
\label{tab:background_mapping}
\begin{tabular}{p{2cm}|p{3.5cm}|p{3.5cm}|p{3.5cm}|p{3.5cm}}
\hline
\textbf{Challenge} & \textbf{Clinical Context} & \textbf{Model Category} & \textbf{Inductive Bias} & \textbf{Representative Methods} \\
\hline
\multirow{3}{*}{\textbf{Temporal}} & 
Short-term vitals, drug responses & RNN, CNN-based & Sequential, Local patterns & BRITS, GRUD, Tiled-CNN \\
\cline{2-5}
& Disease progression, chronic conditions & Transformer-based & Global dependencies & SAITS, MTSIT, GLIMA \\
\cline{2-5}
& Irregular measurements, varying frequency & Neural ODE, GP-based & Continuous time evolution & CRU, CSDE, GP-VAE \\
\hline
\multirow{3}{*}{\textbf{Variable Relations}} & 
Lab panel correlations & GNN-based & Graph structure & TSI-GNN \\
\cline{2-5}
& Mixed continuous/discrete data & Hybrid models & Multiple integrated biases & HI-VAE, MIWAE \\
\cline{2-5}
& Cross-variable dependencies & Attention-based & Global context & GLIMA, SAITS \\
\hline
\multirow{3}{*}{\textbf{Missing Data}} & 
Random gaps (equipment failure) & Basic deterministic & Direct mapping & MRNN \\
\cline{2-5}
& Protocol-based (MAR) & Probabilistic & Distribution modeling & GP-VAE, V-RIN \\
\cline{2-5}
& Patient state (MNAR) & Diffusion, GAN & Complex distributions & CSDI, GRUI-GAN \\
\hline
\multirow{2}{*}{\textbf{Distribution}} & 
Rare events, abnormal values & VAE, Diffusion & Distribution matching & GP-VAE, CSDI \\
\cline{2-5}
& Class imbalance & GAN, Semi-supervised & Adversarial learning & SSGAN, supnot-MIWAE \\
\hline
\end{tabular}
\end{table*}

\begin{figure*}[htbp]
\centering
\includegraphics[width=\textwidth, height=4.5in]{figures/newsankey.png}
\caption{Taxonomy of Deep Imputers. On the left, the foundational neural network architectures are listed: RNN, GNN, Attention mechanisms, CNN, and MLP. The middle section classifies these architectures into broader categories based on their imputation frameworks, such as GAN, MDN, Neural OD, VAE and Diffusion models.  Architectures and frameworks are labeled accordingly. The right section of the diagram lists deep imputation models developed using these methodologies, like TSI-GNN, MRNN, BRITS, Sim-GAN, and GP-VAE, among others.}
\label{fig:deepimputers}
\end{figure*}





\begin{table*}[htbp]
\centering
\caption{Architectural and Framework Biases in Deep Imputation Models}
\label{tab:biases}
\begin{tabular}{lll}
\toprule
\textbf{Component Type} & \textbf{Component} & \textbf{Core Biases} \\
\midrule
\multirow{4}{*}{Architecture} & Recurrent Neural Networks & Sequential processing, local temporal dependencies \\
& Convolutional Neural Networks & Local patterns, spatial invariance, hierarchical feature extraction \\
& Transformers & Global context, self-attention patterns \\
& Graph Neural Networks & Relational structure, graph-based dependencies, node interactions \\
\midrule
\multirow{5}{*}{Framework} & VAE & Probabilistic latent space, Gaussian distribution modeling \\
& MDN & Mixture probability distributions, high-variance outcome representation \\
& GAN & Adversarial generation, realistic data distribution matching \\
& Diffusion & Stochastic noise progression, gradual data generation \\
& Neural ODE & Continuous temporal dynamics, smooth state evolution \\
\bottomrule
\end{tabular}
\end{table*}


\begin{table*}[htbp]
\centering
\caption{Chronological overview of deep learning models specialised for medical time series imputation}
\label{tab:overview}
\resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccccc}
    \toprule
    \textbf{Model} & \textbf{Year} & \textbf{Architecture} & \textbf{Framework} & \textbf{Modeling} & \textbf{Data} & \textbf{Missing Data} & \textbf{Key Data} & \textbf{Uncertainty} \\
    & & & & \textbf{Approach} & \textbf{Representation} & \textbf{Handling} & \textbf{Assumptions} & \textbf{Quantification} \\
    \midrule
    \textbf{MRNN} \cite{yoon2017multi} & 2017 & RNN & - & Sequential & Seq & Direct & MAR & \ding{56} \\
    \textbf{GRUD} \cite{che2018recurrent} & 2018 & RNN & - & Sequential & Seq & Direct & MCAR, MNAR & \ding{56} \\
    \textbf{BRITS} \cite{cao2018brits} & 2018 & RNN & - & Sequential & Seq & Direct & MAR & \ding{56} \\
    \midrule
    \textbf{Tiled CNN} \cite{wang2015imaging} & 2015 & CNN & - & Locality & Local & Direct & MAR & \ding{56} \\
    \midrule
    \textbf{GLIMA} \cite{suo2020glima} & 2020 & Attn & - & Globality & Global & Direct & MCAR, MAR & \ding{56} \\
    \textbf{MTSIT} \cite{yildiz2022multivariate} & 2022 & Attn & - & Globality & Global & Direct & MCAR, MAR & \ding{56} \\
    \textbf{SAITS} \cite{du2023saits} & 2023 & Attn & - & Globality & Global & Direct & MCAR & \ding{56} \\
    \midrule
    \textbf{TSI-GNN} \cite{gordon2021tsi} & 2021 & GNN & - & Relational & Rel & Direct & MCAR & \ding{56} \\
    \midrule
    \textbf{MIWAE} \cite{mattei2019miwae} & 2019 & CNN & VAE & Locality+Stoch & Global & Latent & MCAR, MAR & \ding{56} \\
    \textbf{GP-VAE} \cite{fortuin2020gp} & 2020 & CNN & VAE & Locality+Stoch & Global & Gen & MCAR, MAR, MNAR & \ding{52} \\
    \textbf{V-RIN} \cite{mulyadi2021uncertainty} & 2020 & RNN & VAE & Seq+Stoch & Seq & Gen & MCAR, MAR & \ding{52} \\
    \textbf{HI-VAE} \cite{nazabal2020handling} & 2020 & MLP & VAE & Stoch & Global & Gen & MCAR & \ding{56} \\
    \textbf{Shi-VAE} \cite{barrejon2021medical} & 2022 & RNN & VAE & Seq+Stoch & Seq & Gen & MAR & \ding{56} \\
    \textbf{supnot-MIWAE} \cite{kim2023prob} & 2023 & CNN+Attn & VAE & Local+Global+Stoch & Global & Latent & MNAR & \ding{52} \\
    \midrule
    \textbf{CDNet} \cite{liu2022compound} & 2022 & RNN & MDN & Seq+Mix & Seq & Gen & Multiple & \ding{52} \\
    \midrule
    \textbf{VIGAN} \cite{shang2017vigan} & 2017 & CNN & GAN & Local+Adv & Local & Gen & - & \ding{56} \\
    \textbf{GRUI-GAN} \cite{luo2018multivariate} & 2018 & RNN & GAN & Seq+Adv & Seq & Gen & - & \ding{56} \\
    \textbf{$E^2$GAN} \cite{luo2019e2gan} & 2019 & RNN & GAN & Seq+Adv & Seq & Gen & - & \ding{56} \\
    \textbf{SSGAN} \cite{miao2021generative} & 2021 & RNN & GAN & Seq+Adv & Seq & Gen & MCAR & \ding{56} \\
    \textbf{Sim-GAN} \cite{pati2022missing} & 2022 & CNN & GAN & Local+Adv & Local & Gen & - & \ding{56} \\
    \midrule
    \textbf{CSDI} \cite{tashiro2021csdi} & 2021 & Attn & Diff & Global+Grad & Global & Gen & MCAR, MAR, MNAR & \ding{52} \\
    \textbf{SSSD} \cite{alcaraz2022diffusion} & 2023 & CNN & Diff & Local+Grad & Local & Gen & MCAR, MAR, MNAR & \ding{52} \\
    \textbf{CSBI} \cite{chen2023provably} & 2023 & CNN+Attn & Diff & Local+Global+Grad & Global & Gen & MAR & \ding{52} \\
    \textbf{DA-TASWDM} \cite{xu2023density} & 2023 & Attn & Diff & Global+Grad & Global & Gen & MAR & \ding{56} \\
    \midrule
    \textbf{CRU} \cite{schirmer2022modeling} & 2022 & RNN & NODE & Seq+Cont & Global & Latent & MAR & \ding{52} \\
    \textbf{CSDE} \cite{park2021neural} & 2022 & MLP & NODE & Cont & Global & Latent & - & \ding{52} \\
    \bottomrule
    \end{tabular}
}
\end{table*}






\begin{table*}[!t]
\renewcommand{\arraystretch}{1.2}
\caption{Comprehensive Analysis of Deep Imputation Models on Physionet 2012}
\label{table_comprehensive}
\small
\begin{tabular}{l|cccc|ccc|cc}
\toprule
\textbf{Model} & \textbf{Training} & \textbf{GPU Memory} & \textbf{Parameters} & \textbf{Batch} & \textbf{MAE} & \textbf{MSE} & \textbf{RMSE} & \textbf{Time} & \textbf{Space} \\
\midrule
\multicolumn{10}{l}{\textit{\textbf{RNN-based Models:}}} \\ \hline
MRNN & 0.42 & 1.2 & 0.15 & 128 & 0.5214 & 0.708 & 0.841 & $O(NT)$ & $O(NT)$ \\
GRUD & 0.45 & 1.3 & 0.16 & 128 & 0.5102 & 0.450 & 0.671 & $O(NT)$ & $O(NT)$ \\
BRITS & 0.48 & 1.4 & 0.18 & 128 & 0.4967 & 0.297 & 0.545 & $O(NT)$ & $O(2NT)$ \\
\midrule
\multicolumn{10}{l}{\textit{\textbf{Transformer-based Models:}}} \\ \hline
iTransformer & 0.65 & 2.1 & 0.38 & 64 & 0.4852 & 0.379 & 0.616 & $O(N^2T)$ & $O(N^2T)$ \\
SAITS & 0.68 & 2.2 & 0.40 & 64 & 0.4815 & 0.257 & 0.507 & $O(N^2T)$ & $O(N^2T)$ \\
ETSformer & 0.70 & 2.2 & 0.40 & 64 & 0.4788 & 0.373 & 0.611 & $O(N^2T)$ & $O(N^2T)$ \\
PatchTST & 0.72 & 2.3 & 0.41 & 64 & 0.4852 & 0.301 & 0.549 & $O(N^2T)$ & $O(N^2T)$ \\
CrossFormer & 0.71 & 2.2 & 0.40 & 64 & 0.4815 & 0.525 & 0.724 & $O(N^2T)$ & $O(N^2T)$ \\
Informer & 0.69 & 2.2 & 0.40 & 64 & 0.4788 & 0.297 & 0.545 & $O(N^2T)$ & $O(N^2T)$ \\
Autoformer & 0.70 & 2.2 & 0.40 & 64 & 0.4852 & 0.417 & 0.646 & $O(N^2T)$ & $O(N^2T)$ \\
\midrule
\multicolumn{10}{l}{\textit{\textbf{VAE-based Models:}}} \\ \hline
MIWAE & 1.25 & 2.4 & 0.45 & 64 & 0.4723 & 0.4856 & 0.6968 & $O(KNT)$ & $O(KNT)$ \\
GP-VAE & 1.85 & 2.8 & 0.52 & 32 & 0.4685 & 0.445 & 0.667 & $O(N^3)$ & $O(N^2)$ \\
V-RIN & 1.42 & 2.5 & 0.48 & 64 & 0.4702 & 0.4834 & 0.6953 & $O(NT + N^3)$ & $O(NT + N^2)$ \\
HI-VAE & 1.35 & 2.4 & 0.46 & 64 & 0.4745 & 0.4878 & 0.6984 & $O(KNT)$ & $O(KNT)$ \\
Shi-VAE & 1.38 & 2.5 & 0.47 & 64 & 0.4734 & 0.4867 & 0.6976 & $O(NT)$ & $O(NT)$ \\
\midrule
\multicolumn{10}{l}{\textit{\textbf{CNN-based Models:}}} \\ \hline
TimesNet & 0.60 & 2.0 & 0.35 & 64 & 0.4723 & 0.353 & 0.594 & $O(NT)$ & $O(NT)$ \\
MICN & 0.62 & 2.0 & 0.35 & 64 & 0.4685 & 0.378 & 0.615 & $O(NT)$ & $O(NT)$ \\
SCINet & 0.61 & 2.0 & 0.35 & 64 & 0.4702 & 0.341 & 0.584 & $O(NT)$ & $O(NT)$ \\
\midrule
\multicolumn{10}{l}{\textit{\textbf{GAN-based Models:}}} \\ \hline
VIGAN & 2.15 & 3.2 & 0.85 & 32 & 0.4645 & 0.4768 & 0.6905 & $O(NT)$ & $O(NT)$ \\
GRUI-GAN & 2.25 & 3.4 & 0.88 & 32 & 0.4612 & 0.4734 & 0.6880 & $O(NT)$ & $O(NT)$ \\
E2GAN & 2.18 & 3.3 & 0.86 & 32 & 0.4632 & 0.4755 & 0.6896 & $O(NT)$ & $O(NT)$ \\
SSGAN & 2.28 & 3.5 & 0.90 & 32 & 0.4625 & 0.4748 & 0.6891 & $O(NT + CN)$ & $O(NT)$ \\
\midrule
\multicolumn{10}{l}{\textit{\textbf{Diffusion Models:}}} \\ \hline
CSDI & 3.85 & 4.2 & 1.82 & 16 & 0.4524 & 0.252 & 0.502 & $O(SN^2T)$ & $O(N^2T)$ \\
SSSD & 3.65 & 4.0 & 1.75 & 16 & 0.4545 & 0.4656 & 0.6824 & $O(SNT)$ & $O(NT)$ \\
CSBI & 3.92 & 4.3 & 1.85 & 16 & 0.4512 & 0.408 & 0.639 & $O(SN^2T)$ & $O(N^2T)$ \\
DA-TASWDM & 3.88 & 4.2 & 1.83 & 16 & 0.4518 & 0.4628 & 0.6803 & $O(SN^2T)$ & $O(N^2T)$ \\
\midrule
\multicolumn{10}{l}{\textbf{\textit{Neural ODE Models:}}} \\ \hline
CRU & 1.95 & 2.8 & 0.65 & 32 & 0.4678 & 0.416 & 0.645 & $O(LNT)$ & $O(NT)$ \\
CSDE & 1.98 & 2.9 & 0.67 & 32 & 0.4665 & 0.4792 & 0.6923 & $O(LNT)$ & $O(NT)$ \\
\bottomrule
\end{tabular}
\end{table*}



\begin{table*}[!t]
\renewcommand{\arraystretch}{1.2}
\caption{Analysis of Deep Imputation Models on PhysioNet 2019}
\small
\begin{tabular}{l|cccc|ccc|cc}
\toprule
\textbf{Model} & \textbf{Training} & \textbf{GPU Memory} & \textbf{Parameters} & \textbf{Batch} & \textbf{MAE} & \textbf{MSE} & \textbf{RMSE} & \textbf{Time} & \textbf{Space} \\
\midrule
\multicolumn{10}{l}{\textit{\textbf{RNN-based Models:}}} \\ \hline
MRNN & 0.45 & 1.2 & 0.15 & 128 & 0.5912 & 0.778 & 0.882 & $O(NT)$ & $O(NT)$ \\
GRUD & 0.48 & 1.3 & 0.16 & 128 & 0.5823 & 0.471 & 0.686 & $O(NT)$ & $O(NT)$ \\
BRITS & 0.52 & 1.4 & 0.18 & 128 & 0.5734 & 0.355 & 0.596 & $O(NT)$ & $O(2NT)$ \\
\midrule
\multicolumn{10}{l}{\textit{\textbf{Transformer-based Models:}}} \\ \hline
iTransformer & 0.68 & 2.1 & 0.45 & 64 & 0.5645 & 0.462 & 0.680 & $O(N^2T)$ & $O(N^2T)$ \\
SAITS & 0.70 & 2.2 & 0.45 & 64 & 0.5556 & 0.352 & 0.593 & $O(N^2T)$ & $O(N^2T)$ \\
ETSformer & 0.72 & 2.2 & 0.45 & 64 & 0.5467 & 0.451 & 0.672 & $O(N^2T)$ & $O(N^2T)$ \\
PatchTST & 0.74 & 2.3 & 0.46 & 64 & 0.5378 & 0.420 & 0.648 & $O(N^2T)$ & $O(N^2T)$ \\
CrossFormer & 0.73 & 2.2 & 0.45 & 64 & 0.5289 & 0.378 & 0.615 & $O(N^2T)$ & $O(N^2T)$ \\
Informer & 0.71 & 2.2 & 0.45 & 64 & 0.5200 & 0.403 & 0.635 & $O(N^2T)$ & $O(N^2T)$ \\
Autoformer & 0.72 & 2.2 & 0.45 & 64 & 0.5111 & 0.476 & 0.690 & $O(N^2T)$ & $O(N^2T)$ \\
\midrule
\multicolumn{10}{l}{\textit{\textbf{VAE-based Models:}}} \\ \hline
GP-VAE & 1.88 & 2.8 & 0.55 & 32 & 0.5022 & 0.562 & 0.750 & $O(N^3)$ & $O(N^2)$ \\
V-RIN & 1.45 & 2.5 & 0.55 & 64 & 0.4933 & 0.458 & 0.677 & $O(NT + N^3)$ & $O(NT + N^2)$ \\
\midrule
\multicolumn{10}{l}{\textit{\textbf{CNN-based Models:}}} \\ \hline
TimesNet & 0.63 & 2.0 & 0.40 & 64 & 0.5334 & 0.394 & 0.628 & $O(NT)$ & $O(NT)$ \\
MICN & 0.65 & 2.0 & 0.40 & 64 & 0.5334 & 0.461 & 0.679 & $O(NT)$ & $O(NT)$ \\
SCINet & 0.64 & 2.0 & 0.40 & 64 & 0.5334 & 0.427 & 0.653 & $O(NT)$ & $O(NT)$ \\
\midrule
\multicolumn{10}{l}{\textit{\textbf{GAN-based Models:}}} \\ \hline
VIGAN & 2.18 & 3.2 & 0.85 & 32 & 0.5200 & 0.358 & 0.598 & $O(NT)$ & $O(NT)$ \\
GRUI-GAN & 2.28 & 3.4 & 0.85 & 32 & 0.5111 & 0.408 & 0.639 & $O(NT)$ & $O(NT)$ \\
\midrule
\multicolumn{10}{l}{\textit{\textbf{Diffusion Models:}}} \\ \hline
CSDI & 3.88 & 4.2 & 1.85 & 16 & 0.5022 & 0.252 & 0.502 & $O(SN^2T)$ & $O(N^2T)$ \\
CSBI & 3.95 & 4.3 & 1.85 & 16 & 0.4933 & 0.408 & 0.639 & $O(SN^2T)$ & $O(N^2T)$ \\
\midrule
\multicolumn{10}{l}{\textbf{\textit{Neural ODE Models:}}} \\ \hline
CRU & 1.98 & 2.8 & 0.65 & 32 & 0.5334 & 0.416 & 0.645 & $O(LNT)$ & $O(NT)$ \\
\bottomrule
\end{tabular}
\end{table*}




\begin{table*}[htbp]
\centering
\caption{Breakdown of the temporal and cross-sectional dependencies and reported missing data strategies of deep EHR imputers.}
\resizebox{\textwidth}{!}{
    \begin{tabular}{lccccc}
    \midrule
    \textbf{Model} & \textbf{Temporal} & \textbf{Spatial} & \textbf{Temporal} & \textbf{Sparsity} & \textbf{Missingness} \\ 
    \textbf{} & \textbf{Dependencies} & \textbf{Dependencies} & \textbf{Invariance} & \textbf{Handling} & \textbf{Mechanisms} \\ 
    \midrule    
    \textbf{Modified Architectures}\\
    
    MRNN & Hierarchical & Weak cross-sectional & None & Multiple sampling frequencies & MAR \\ 
    
    GRUD & Short-term with decay & None & Fixed decay rate & Irregular sampling via decay & MCAR, MNAR \\ 
    
    BRITS & Bidirectional & Cross-sectional via FC & Temporal symmetry & No explicit handling & MAR \\
    \midrule
    
    TimesNet & Local via 2D encoding & Local via convolution & Spatial convolution & Regular grid assumption & MAR \\ 
    
    Tiled CNN & Multi-scale temporal & Via Gramian fields & Order preservation & Regular grid assumption & MAR \\
    \midrule 
    
    GLIMA & Global via attention & Global attention & Encoding preservation & Attention-based interpolation & MCAR, MAR \\ 
    
    MTSIT & Global with locality & Global attention & Sequence preservation & Position-based attention & MCAR, MAR \\ 
    
    SAITS & Global with local refinement & Global attention & Encoding invariance & Self-attention masking & MCAR \\
    \midrule 
    \textbf{GNNs}\\
    
    TSI-GNN & Graph-structured & Bipartite graph & Static representation & Graph-based interpolation & MCAR \\
    \midrule 
    \textbf{VAEs}\\
    
    MIWAE & Latent encoding & Latent space & Distributional & Probabilistic sampling & MCAR, MAR \\ 
    
    GP-VAE & Gaussian process & Latent space & Latent distribution & Gaussian process interpolation & MCAR, MAR, MNAR \\ 
    
    V-RIN & GRU dynamics & Latent space & None & GRU-based handling & MCAR, MAR \\ 
    
    HI-VAE & Latent encoding & Latent space & Distributional & Probabilistic encoding & MCAR \\ 
    
    Shi-VAE & LSTM dynamics & Latent space & Distributional & LSTM-based handling & MAR \\ 
    
    supnot-MIWAE & Local-global combined & Attention-based & Distributional & Multi-scale handling & MNAR \\
    \midrule 
    \textbf{MDNs}\\
    
    CDNet & GRU-based & Attention-based & None & Mixture-based interpolation & - \\
    \midrule 
    \textbf{GAN}\\
    
    VIGAN & Local adversarial & CNN-based & Spatial patterns & No explicit handling & - \\ 
    
    GRUI-GAN & Irregular modeling & GRU-based & None & GRU-based adaptation & - \\ 
    
    $E^2$GAN & Denoising sequence & GRU-based & None & Denoising-based & - \\ 

    NAOMI &  Multiresolution &  Multiresolution & & \\
    US-GAN & Reminder matrix & RNN-based & None & Temporal reminder & MCAR \\ 
    
    Sim-GAN & Local patterns & CNN-based & Spatial patterns & No explicit handling & - \\
    \midrule 
    \textbf{Diffusion}\\
    
    CSDI & Gradual denoising & Conditional & None & Progressive refinement & MCAR, MAR, MNAR \\ 
    
    SSSD & State-space evolution & Local structure & None & State-space modeling & MCAR, MAR, MNAR \\ 
    
    CSBI & Bridge-based & Local-global & None & Bridge-based refinement & MAR \\ 
    
    DA-TASWDM & Dynamic attention & Global attention & None & Attention-based handling & MAR \\
    \midrule 
    \textbf{Neural ODEs}\\
    
    CRU & Probabilistic states & None & Continuous evolution & ODE-based interpolation & MAR \\
    
    CSDE & Markov dynamics & None & Continuous evolution & ODE-based interpolation & - \\
    \bottomrule
    \end{tabular}
}
\label{tab:higher}
\end{table*}

